SIM-Sync: From Certifiably Optimal Synchronization over the 3D Similarity Group to Scene Reconstruction with Learned Depth

This paper presents SIM-Sync, a certifiably optimal algorithm that estimates camera trajectory and 3D scene structure directly from multiview image keypoints. SIM-Sync fills the gap between pose graph optimization and bundle adjustment; the former admits efficient global optimization but requires relative pose measurements and the latter directly consumes image keypoints but is difficult to optimize globally (due to camera projective geometry). The bridge to this gap is a pretrained depth prediction network. Given a graph with nodes representing monocular images taken at unknown camera poses and edges containing pairwise image keypoint correspondences, SIM-Sync first uses a pretrained depth prediction network to lift the 2D keypoints into 3D scaled point clouds, where the scaling of the per-image point cloud is unknown due to the scale ambiguity in monocular depth prediction. SIM-Sync then seeks to synchronize jointly the unknown camera poses and scaling factors (i.e., over the 3D similarity group). The SIM-Sync formulation, despite nonconvex, allows designing an efficient certifiably optimal solver that is almost identical to the SE-Sync algorithm. We demonstrate the tightness, robustness, and practical usefulness of SIM-Sync in both simulated and real experiments. In simulation, we show (i) SIM-Sync compares favorably with SE-Sync in scale-free synchronization, and (ii) SIM-Sync can be used together with robust estimators to tolerate a high amount of outliers. In real experiments, we show (a) SIM-Sync achieves similar performance as Ceres on bundle adjustment datasets, and (b) SIM-Sync performs on par with ORB-SLAM3 on the TUM dataset with zero-shot depth prediction.

==> sections/fig-simsync-overview.tex <==
%!TEX root = ../main.tex

\begin{figure}[t]
    \centering
    \includegraphics[width= 1.0\columnwidth]{figures/Cover_vis.png}
    \caption{Illustration of \simsync on the \tum dataset~\cite{sturm2012benchmark}.}
    \label{SIM-Sync_vis}
\end{figure}


==> sections/related-work.tex <==
%!TEX root = ../main.tex
\section{Related Work}
\label{sec:related-work}

We review related work on structure from motion and visual SLAM in Section \ref{sec:related-work:vision}, and on certifiable geometric perception in Section \ref{sec:related-work:certifiable}.

\subsection{Structure from Motion and SLAM}
\label{sec:related-work:vision}
Estimating camera poses and scene structure from sensor data is a long-standing problem in computer vision and robotics. This problem is variously called structure from motion (SfM) \cite{schonberger2016structure} or simultaneous localization and mapping (SLAM) \cite{cadena16tro-past}, where SLAM can often rely on GPS, IMU, and even wireless communication~\cite{jadhav22ijrr-wireless}. 
In classic SfM and SLAM, the problem is typically decomposed into feature matching and geometric estimation, where feature matching establishes keypoint correspondences between images (and point clouds) and geometric estimation seeks to find the best poses and structure that fit the correspondences. Feature matching, closely related to representation learning, is one of the most popular topics in computer vision with a vast amount of literature, for which we refer to \cite{image-matching-challenge} for a recent review. When it comes to geometric estimation, as introduced in Section \ref{sec:introduction}, two popular paradigms are the pose graph optimization formulation in SLAM and the bundle adjustment formulation in SfM.

Recently, a number of methods seek to integrate learned components into classic SfM or SLAM methods. \cite{mahjourian2018unsupervised} explored jointly optimizing depth maps, camera poses and confidence masks for weighting the photo-metric loss during training. \cite{zhou2017unsupervised} learns depth and ego-motion from monocular video without supervision. 
\cite{yang2020d3vo} leverages modules for learned prediction of depth, pose, and uncertainty within a bundle adjustment framework. 
DROID-SLAM~\cite{teed2021droid} makes use of a dense bundle adjustment layer to update depth map and camera poses concurrently. 
\cite{merrillfast} leverages pre-trained depth prediction for better initialization of visual inertial odometry. 

In this work, we use a pretrained depth prediction network to lift 2D image keypoints as 3D scaled point clouds to enable global synchronization of camera poses and unknown scaling coefficients in depth prediction.


\subsection{Certifiably Optimal Geometric Perception}
\label{sec:related-work:certifiable}
Certifiably optimal geometric perception refers to developing algorithms that either solve geometric estimation problems to global optimality and produce an optimality certificate, or fail to do so but provide a bound of suboptimality~\cite[Definition 1]{yang2022certifiably}.
Semidefinite programming has been the major tool for developing certifiably optimal estimation algorithms. 
The pioneering work by Kahl and Henrion~\cite{kahl2007globally} employs Lasserre's hierarchy to tackle various early perception problems, including camera resectioning, homography estimation, and fundamental matrix estimation. More recently, certifiable algorithms have been developed for modern applications such as outlier-robust estimation \cite{yang2022certifiably, yang2020one}, pose graph optimization \cite{carlone2016planar, rosen2019se}, rotation averaging \cite{eriksson2018rotation, fredriksson2012simultaneous}, triangulation \cite{aholt2012qcqp,cifuentes2021convex}, 3D registration \cite{yang2020teaser, briales2017convex, chaudhury2015global, iglesias2020global, maron2016point}, absolute pose estimation \cite{agostinho2023cvxpnpl}, relative pose estimation \cite{briales2018certifiably, garcia2021certifiable, zhao2020efficient}, hand-eye calibration \cite{giamou2019certifiably, heller2014hand, wise2020certifiably}, uncertainty propagation in non-rigid SfM \cite{song2022closed} and category-level object perception \cite{shi2021optimal, yang2020perfect}.

In this work, we develop the first certifiably optimal algorithm that estimates 3D scene and camera poses directly from 2D image correspondences.

